Simultaneously enhancing brightness and purity of WSe$_2$ single photon emitter using high-aspect-ratio nanopillar array on metal

Monolayer semiconductor transferred on nanopillar arrays provides site-controlled, on-chip single photon emission, which is a scalable light source platform for quantum technologies. However, the brightness of these emitters reported to date often falls short of the perceived requirement for such applications. Also, the single photon purity usually degrades as the brightness increases. Hence, there is a need for a design methodology to achieve enhanced emission rate while maintaining high single photon purity. Using WSe$_2$ on high-aspect-ratio ($\sim 3$ - at least two-fold higher than previous reports) nanopillar arrays, here we demonstrate $>10$ MHz single photon emission rate in the 770-800 nm band that is compatible with quantum memory and repeater networks (Rb-87-D1/D2 lines), and satellite quantum communication. The emitters exhibit excellent purity (even at high emission rates) and improved out-coupling due to the use of a gold back reflector that quenches the emission away from the nanopillar.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
